Quasi-equilibrium models for triaxially deformed rotating compact stars

Quasi-equilibrium models of rapidly rotating triaxially deformed stars are computed in general relativistic gravity, assuming a conformally flat spatial geometry (Isenberg-Wilson-Mathews formulation) and a polytropic equation of state. Highly deformed solutions are calculated on the initial slice covered by spherical coordinate grids, centered at the source, in all angular directions up to a large truncation radius. Constant rest mass sequences are calculated from nearly axisymmetric to maximally deformed triaxial configurations. Selected parameters are to model (proto-) neutron stars; the compactness is M/R = 0.001, 0.1, 0.14, 0.2 for polytropic index n = 0.3 and M/R = 0.001, 0.1, 0.12, 0.14 for n = 0.5. We confirmed that the triaxial solutions exist for these parameters as in the case of Newtonian polytropes. However, it is also found that the triaxial sequences become shorter for higher compactness, and those may disappear at a certain large compactness for the n = 0.5 case. In the scenario of the contraction of proto-neutron stars being subject to strong viscosity and rapid cooling, it is plausible that, once the viscosity driven secular instability sets in during the contraction, the proto-neutron stars are always maximally deformed triaxial configurations, as long as the compactness and the equation of state parameters allow such triaxial sequences. Detection of gravitational waves from such sources may be used as another probe for the nuclear equation of state.

==> reference.tex <==
    Nikolaos Stergioulas,
    "Rotating Stars in Relativity",
    Living Rev. Relativity 6,  (2003),  3. URL (cited on <date>):
    http://www.livingreviews.org/lrr-2003-3 

The date given as <date> then uniquely identifies the version of 
the article you are referring to. 
%
% note: this record is encoded in utf-8! to use it with tex, you may have to
% adapt the encoding (using the tools 'recode' or 'iconv') or use the latex
% ucs package (http://ctan.tug.org/tex-archive/macros/latex/contrib/unicode/)
%
@article{lrr-2003-3,
  title    = {Rotating Stars in Relativity},
  author   = {Nikolaos Stergioulas},
  journal  = {Living Reviews in Relativity},
  year     = {2003},
  number   = {3},
  volume   = {6},
  keywords = {relativistic stars, rotation, stability, oscillations, numerical relativity},
  url      = {http://www.livingreviews.org/lrr-2003-3}
}

--

James, R.A., ``The Structure and Stability of Rotating Gas Masses'', 
Astrophys. J., 140, 552-582, (1964).

@article{349,
  author   = {James, R.A.},
  format   = {print},
  journal  = {Astrophys. J.},
  keywords = {Astrophysics, Instability, Rotation},
  pages    = {552--582},
  refdb_id = {http://relativity.livingreviews.org/refdb/record/349},
  title    = {The Structure and Stability of Rotating Gas Masses},
  volume   = {140},
  year     = {1964}
}

--

Skinner, D., and Lindblom, L., ``On the Viscosity-driven Secular Instability in Rotating Neutron Star'', 
Astrophys. J., 461, 920-926, (1996).

@article{350,
  author   = {Skinner, D. and Lindblom, L.},
  format   = {print},
  journal  = {Astrophys. J.},
  keywords = {Instability, Neutron stars, Rotation},
  pages    = {920--926},
  refdb_id = {http://relativity.livingreviews.org/refdb/record/350},
  title    = {On the Viscosity-driven Secular Instability in Rotating Neutron Star},
  volume   = {461},
  year     = {1996}
}

--

Bonazzola, S. Frieben, J., and Gourgoulhon, E., ``Spontaneous Symmetry Breaking of Rapidly Rotating Stars in General Relativity: Influence of the 3D-shift Vector'', 
Astron. Astrophys., 331, 280-290, (1998).

@article{351,
  author   = {Bonazzola, S. and Frieben, J. and Gourgoulhon, E.},
  format   = {print},
  journal  = {Astron. Astrophys.},
  keywords = {Instability, Relativistic stars, Rotation},
  pages    = {280--290},
  refdb_id = {http://relativity.livingreviews.org/refdb/record/351},
  title    = {Spontaneous Symmetry Breaking of Rapidly Rotating Stars in General Relativity: Influence of the 3D-shift Vector},
  volume   = {331},
  year     = {1998}
}

--

S. Bonazzola, et al., ``Spontaneous Symmetry Breaking of Rapidly Rotating Stars in General Relativity'',

--

Shapiro, S.L., and Zane, S., ``Bar Mode Instability in Relativistic Rotating Stars: 
A Post-Newtonian Treatment'', Astrophys. J., 460, 379-389, (1996). 
@article{369,
  author   = {Shapiro, S.L. and Zane, S.},
  format   = {print},
  journal  = {Astrophys. J.},
  keywords = {Instability, Post-Newtonian approximations, Relativistic stars},
  pages    = {379--389},
  refdb_id = {http://relativity.livingreviews.org/refdb/record/369},
  title    = {Bar Mode Instability in Relativistic Rotating Stars: A Post-Newtonian Treatment},
  volume   = {460},
  year     = {1996}
}
--
Di Girolamo, T., and Vietri, M., ``Post-Newtonian Treatment of Bar Mode Instability in Rigidly Rotating Equilibrium Configurations for Polytropic Stars'', Astrophys. J., 581, 519-549, (2002). For a related online version see: T. Di Girolamo, et al., ``Post-Newtonian treatment of bar mode instability in rigidly rotating equilibrium configurations for neutron stars'', (May, 2002),
@article{522,
  author   = {Di Girolamo, T. and Vietri, M.},
  format   = {print},
  journal  = {Astrophys. J.},
  keywords = {Instability, Neutron stars, Post-Newtonian approximations},
  pages    = {519--549},
  refdb_id = {http://relativity.livingreviews.org/refdb/record/522},
  title    = {Post-Newtonian Treatment of Bar Mode Instability in Rigidly Rotating Equilibrium Configurations for Polytropic Stars},
  volume   = {581},
  year     = {2002}
}
--
Gondek-Rosinska, D., and E., Gourgoulhon, 
``Jacobi-like bar mode instability of relativistic rotating bodies'', 
Phys. Rev. D, 66, 044021-1-044021-11, (2002). 
@article{523,
  author   = {Gondek-Rosi{\'{n}}ska, D. and Gourgoulhon, E.},
  format   = {print},
  id       = {044021},
  journal  = {Phys. Rev. D},
  keywords = {Instability, Relativistic stars, Viscosity},
  pages    = {1--11},
  refdb_id = {http://relativity.livingreviews.org/refdb/record/523},
  title    = {Jacobi-like bar mode instability of relativistic rotating bodies},
  volume   = {66},
  year     = {2002}
}

Gondek-Rosinska, D., Gourgoulhon, E., and Haensel, P., 
``Rapidly Rotating Strange Quark Stars as Sources of Gravitational Waves'', 
preprint, submitted to Astron. Astrophys., (2003).
@unpublished{538,
  author   = {Gondek-Rosi{\'{n}}ska, D. and Gourgoulhon, E. and Haensel, P.},
  format   = {submitted},
  journal  = {Astron. Astrophys.},
  keywords = {Equation of state, Gravitational waves, Relativistic stars},
  refdb_id = {http://relativity.livingreviews.org/refdb/record/538},
  title    = {Rapidly Rotating Strange Quark Stars as Sources of Gravitational Waves},
  year     = {2003}
}

